Whitening-based Contrastive Learning of Sentence Embeddings

This paper presents a whitening-based contrastive learning method for sentence embedding learning (WhitenedCSE), which combines contrastive learning with a novel shuffled group whitening. Generally, contrastive learning pulls distortions of a single sample (i.e., positive samples) close and push negative samples far away, correspondingly facilitating the alignment and uniformity in the feature space. A popular alternative to the "pushing'' operation is whitening the feature space, which scatters all the samples for uniformity. Since the whitening and the contrastive learning have large redundancy w.r.t. the uniformity, they are usually used separately and do not easily work together. For the first time, this paper integrates whitening into the contrastive learning scheme and facilitates two benefits. 1) Better uniformity. We find that these two approaches are not totally redundant but actually have some complementarity due to different uniformity mechanism. 2) Better alignment. We randomly divide the feature into multiple groups along the channel axis and perform whitening independently within each group. By shuffling the group division, we derive multiple distortions of a single sample and thus increase the positive sample diversity. Consequently, using multiple positive samples with enhanced diversity further improves contrastive learning due to better alignment. Extensive experiments on seven semantic textual similarity tasks show our method achieves consistent improvement over the contrastive learning baseline and sets new states of the art, e.g., 78.78\% (+2.53\% based on BERT\ba) Spearman correlation on STS tasks.

==> figures/mclf.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.99\linewidth]{figures/mclf.pdf}
    \caption{The comparative experiments of different contrastive loss function.}
    \label{fig:mclf}
    \vspace{-5pt}
\end{figure}


==> sections/acknowledgements.tex <==
\section*{Acknowledgements}

This document has been adapted
by Steven Bethard, Ryan Cotterell and Rui Yan
from the instructions for earlier ACL and NAACL proceedings, including those for 
ACL 2019 by Douwe Kiela and Ivan Vuli\'{c},
NAACL 2019 by Stephanie Lukin and Alla Roskovskaya, 
ACL 2018 by Shay Cohen, Kevin Gimpel, and Wei Lu, 
NAACL 2018 by Margaret Mitchell and Stephanie Lukin,
Bib\TeX{} suggestions for (NA)ACL 2017/2018 from Jason Eisner,
ACL 2017 by Dan Gildea and Min-Yen Kan, 
NAACL 2017 by Margaret Mitchell, 
ACL 2012 by Maggie Li and Michael White, 
ACL 2010 by Jing-Shin Chang and Philipp Koehn, 
ACL 2008 by Johanna D. Moore, Simone Teufel, James Allan, and Sadaoki Furui, 
ACL 2005 by Hwee Tou Ng and Kemal Oflazer, 
ACL 2002 by Eugene Charniak and Dekang Lin, 
and earlier ACL and EACL formats written by several people, including
John Chen, Henry S. Thompson and Donald Walker.
Additional elements were taken from the formatting instructions of the \emph{International Joint Conference on Artificial Intelligence} and the \emph{Conference on Computer Vision and Pattern Recognition}.

==> sections/preliminaries.tex <==
\section{Preliminaries}
In this section, 

==> tables/multi_positives.tex <==

\begin{table}[t]
    \begin{center}
    \centering
    \small
    \resizebox{0.88\columnwidth}{!}{%
    \begin{tabular}{lccc}
    \toprule
    \tf{Augmentation Strategy} & & & STS-avg\\
    \midrule
       ~~Dropout (unsup. SimCSE)  & & & 76.25 \\
       ~~Dup+Dropout ~\cite{wu2021esimcse}  & & & 76.73 \\
    \midrule
    \tf{Multi-positives} & & &\\
    ~~k=2 & & & \\
       ~~~~Dropout (unsup. SimCSE)  & & & 76.55 \\
       ~~~~Dup+Dropout ~\cite{wu2021esimcse}  & & & \tf{77.13} \\
    ~~k=3 & & & \\
       ~~~~Dropout (unsup. SimCSE)  & & & 76.58 \\
       ~~~~Dup+Dropout ~\cite{wu2021esimcse}  & & & 77.01 \\
    ~~k=4 & & & \\ 
       ~~~~Dropout (unsup. SimCSE)  & & & \tf{76.64} \\
       ~~~~Dup+Dropout ~\cite{wu2021esimcse}  & & & 77.07 \\
    \bottomrule
    \end{tabular}
    }
    \end{center}

    \caption{
        Comparison of whitening strategy on STS-B development set (Spearman's correlation).
        % \ti{Crop $k$\%}: keep 100-$k$\% of the length;
        % \ti{word deletion $k$\%}: delete $k$\% words;
        % % \ti{delete one word}: randomly delete one word; 
        % \ti{Synonym replacement}: use \texttt{nlpaug}~\cite{ma2019nlpaug} to randomly replace one word with its synonym;
        % \ti{MLM $k$\%}: use BERT\ba~to replace $k$\% of words.
        % All of them include the standard 10\% dropout (except ``w/o dropout'').
    }
    \label{tab:multi_positive}
\end{table}

